Sparse and Continuous Attention Mechanisms

Exponential families are widely used in machine learning; they include many distributions in continuous and discrete domains (e.g., Gaussian, Dirichlet, Poisson, and categorical distributions via the softmax transformation). Distributions in each of these families have fixed support. In contrast, for finite domains, there has been recent work on sparse alternatives to softmax (e.g. sparsemax and alpha-entmax), which have varying support, being able to assign zero probability to irrelevant categories. This paper expands that work in two directions: first, we extend alpha-entmax to continuous domains, revealing a link with Tsallis statistics and deformed exponential families. Second, we introduce continuous-domain attention mechanisms, deriving efficient gradient backpropagation algorithms for alpha in {1,2}. Experiments on attention-based text classification, machine translation, and visual question answering illustrate the use of continuous attention in 1D and 2D, showing that it allows attending to time intervals and compact regions.

==> sparse_families.tex <==
\section{Background}

\subsection{Exponential families}

Exponential families are widely used in statistics \citep{barndorff2014information}. They have the form
\begin{equation}\label{eq:exponential_families}
p_\theta(t) = \exp \bigl(\theta^\top \phi(t) - A(\theta)\bigr),
\end{equation}
where $\phi(t)$ is a vector of \textit{statistics}, $\theta$ is a vector of \textit{canonical parameters}, and $A(\theta) := \log \int_S \exp(\theta^\top\phi(t))$
is the \textit{log-partition function}. 
For finite $S$, this integral is a summation, and by defining $\phi(t) = e_t$ (the Euclidean basis vector) for $t = 1, 2, \ldots, |S|$, we obtain a categorical distribution, which relates to $\theta$ via the {\bf softmax transformation},
\[
p_\theta(t) = [\mathrm{softmax}(\theta)]_t = \tfrac{\exp(\theta_t)}{\sum_{k=1}^{|S|} \exp(\theta_k)} \in \triangle,
\]
where $\triangle$ is the $|S|-$dimensional probability simplex.

\andre{need to adjust below}
For continuous domains with $\nu$ being the Lebesgue measure, some notable examples for particular choices of $f$ follow.

\begin{example} \label{ex:Gaussian}Let $S=\mathbb{R}^N$, $\Sigma \in \mathbb{R}^{N\!\times\! N}$ be symmetric positive definite, and $f(t) \!=\!  \tfrac{-1}{2} (t\!-\!\mu)^\top\Sigma^{-1}(t\!-\!\mu)$. This leads to a multivariate Gaussian, $\hat{p}_{\Omega}[f](t) = \mathcal{N}(t; \mu, \Sigma)$, with Shannon negentropy $\Omega(p) = -\frac{1}{2}\log \det (2\pi e \Sigma)$.
For $N=1$ and $\Sigma = \sigma^2$, we obtain a univariate Gaussian $\mathcal{N}(t; \mu, \sigma^2)$.
\end{example}

\begin{example}For $S=\mathbb{R}$ and $f(t) = -|t-\mu|/b$, we get a Laplace density, $\hat{p}_{\Omega}[f](t) = \tfrac{1}{2b}\exp\left(-|t-\mu|/b\right)$, with Shannon negentropy $\Omega(p) = -\log(2b e)$.
\end{example}

Note that in both Examples 1 and 2, $f(t)\leq 0$, thus  $f\in \mathcal{F}$. 

\andre{categorical with softmax, (multivariate) Gaussian, Laplace}

\andre{connection with Shannon-Boltzmann-Gibbs via the maxent principle and the variational free energy principle}

\andre{nice properties}

%\subsection{Shannon's negentropy}

For the Shannon's negentropy $\Omega(p) = \int_S p(t)\log p(t)$, the corresponding $\Omega$-RPM recovers Boltzmann-Gibbs distributions (\citet{cover2012elements}; see App.~\ref{sec:diff_ent_exp_family}): 
\begin{equation}\label{eq:boltzmann}
\hat{p}_\Omega[f](t)\!=\!\frac{\exp(f(t))}{\int_S \exp(f(t'))d\nu(t')}\!=\!\exp \bigl(f(t) - A(f)\bigr),
\end{equation}
where 
$A(f) := \log \int_S \exp(f(t))$
is the log-partition function. 
For finite $S$, this integral is a summation and we can write $f$ as a vector, $f = [f_1, \ldots, f_{|S|}] \in \mathbb{R}^{|S|}$. In this case, the $\Omega$-RPM is the {\bf softmax transformation},
\[
\hat{p}_\Omega[f] = \mathrm{softmax}(f) = \tfrac{\exp(f)}{\sum_{k=1}^{|S|} \exp(f_k)} \in \triangle,
\]
where $\triangle$ is the $|S|-$dimensional probability simplex.




\subsection{Tsallis statistics}

generalization of log and exp

definition of Tsallis entropy

$q$-exponential families

widely used in statistical physics to model heavy-tailed distributions

also used in ML: $t$-student distribution

``deformed exponential families'' \citep{naudts2009q,sears2010generalized}, also called  $q$-exponential families \citep{matsuzoe2012geometry}

used in machine learning by \citep{ding2010t} (under the name 
``$t$-exponential families'') to model heavy tail distributions. 

Unlike those prior works, we are interested in the sparse, light tail scenario ($\alpha>1$), not in heavy tails.

Geometry of Tsallis $q$-entropy has been studied by 
\citet[\S 4.3]{amari2016information}. This $q$ equals $2-\alpha$ in our notation and $\alpha = 2q - 1$ in Amari's notation.

Central in this context are the notions of  $\beta$-logarithm and $\beta$-exponential  \citep{Tsallis1988}, generalizing the standard logarithm and exponential functions. The first, $\log_{\beta}: \mathbb{R}_{++} \rightarrow \mathbb{R}$ (not to be confused with base-$\beta$ logarithm), is defined as
\begin{equation}\label{eq:beta_log}
    \log_{\beta}(u) = \left\{
    \begin{array}{ll}
        \frac{u^{1-\beta} - 1}{1-\beta}, & \beta \ne 1 \\
        \log u, & \beta = 1;
    \end{array}
    \right.
\end{equation}
the latter, $\exp_{\beta}: \mathbb{R} \rightarrow \mathbb{R}$, is its inverse, ($\exp_{\beta}(\ln_{\beta}(u)) = u$)
\begin{equation}\label{eq:beta_exp}
    \exp_{\beta}(u) = \left\{
    \begin{array}{ll}
     	[1 + (1-\beta)u]_+^{1/(1-\beta)}, & \beta \ne 1 \\
        \exp u, & \beta = 1.
    \end{array}
    \right.
\end{equation}
Note that ${\displaystyle \lim_{\beta \rightarrow 1}}\ln_\beta(u) = \ln u$ and ${\displaystyle\lim_{\beta \rightarrow 1}}\exp_\beta(u) = \exp(u)$, and that the $\alpha$-Tsallis negentropy can be written as
\begin{eqnarray*}
\Omega_\alpha(p) = \frac{1}{\alpha} \mathbb{E}_{p}[\log_{2-\alpha}(p(t))] = \frac{1}{\alpha} \! \int_S \! p(t)^\alpha \log_{\alpha}(p(t)).
\end{eqnarray*}

The {\bf $\alpha$-Tsallis negentropies}  \citep{havrda1967quantification,Tsallis1988} are defined as:
\begin{equation}\label{eq:tsallis}
\Omega_{\alpha}(p) =
\begin{cases}
\frac{1}{\alpha(\alpha-1)}\left( \int_S  p(t)^\alpha - 1 \right), &
\alpha \ne 1,\\
\int_S p(t) \log p(t), &
\alpha = 1.
\end{cases}
\end{equation}

\andre{however, it would be good to explain (or mention) the difference, because dropping the $1/\alpha$ factor is more common in the literature. Moreover, the equation is a bit unclear, because it is unclear whether the 1 is inside the integral or outside of it. This confusion stems from the choice to drop the dx terms (or dnu terms according to your notation). If it were inside the integral, the integral would go to infty though, so that wouldn't make sense.}

This family is continuous, \textit{i.e.}, $\lim_{\alpha \rightarrow
1}\Omega_{\alpha}(p) = \Omega_{1}(p)$, for any $p \in \mathcal{M}_+^1(S)$, with $\Omega_{1}(p)$ recovering Shannon's negentropy (proof in App.~\ref{sec:gini_ent_sparse_family}). Another notable case is $\Omega_2(p)$,
\begin{equation}\label{eq:gini}
{\textstyle \Omega_2(p) = \tfrac{1}{2}\int_S p(t)^2  - \tfrac{1}{2},}
\end{equation}
the negative of which has several names, {\it e.g.}, Gini-Simpson index \citep{Jost2006} or Rao's quadratic entropy \citep{Rao1982}.



\citet{blondel2020learning}  showed that, for finite $S$,  $\Omega_2$-RPM is the {\bf sparsemax} transformation, $\hat{p}_\Omega[f] = \mathrm{sparsemax}(f) =
\arg\min_{p \in \triangle} \|p - f\|^2$
(Euclidean projection of  $f\in\mathbb{R}^{|S|}$ onto the $|S|$-dimensional probability simplex $\triangle$). Other values of $\alpha$ were studied by \citet{peters2019sparse}, under the name {\bf $\alpha$-entmax} transformation. For $\alpha>1$, these transformations tend to return sparse distributions, where several entries have zero probability. This raises the question of whether similar properties can be obtained when $S$ is continuous. The following proposition (proof in  App.~\ref{sec:gini_ent_sparse_family}) answers this question by providing a general expression for $\Omega_{\alpha}$-RPM.  A key observation is that $\Omega_{\alpha}$ is strictly convex, for any $\alpha > 0$, thus satisfying the condition in Def.~\ref{def:regularized_prediction}.



\section{Sparse Families}\label{sec:sparse_families}

\subsection{Regularized prediction maps}

\andre{point relation to variational free energy principle}

\citet{blondel2020learning} introduced $\Omega$-regularized prediction maps for the case where $S$ is finite. This is a general framework for mapping $|S|$-dimensional real vectors (\textit{e.g.}, label scores computed by a neural network) into probability vectors in the simplex, with a regularizer $\Omega$ encouraging uniform distributions. Particular choices of $\Omega$ recover well-known transformations such as softmax \citep{bridle1990probabilistic}, sparsemax \citep{Martins2016ICML}, and others. We extend that framework to arbitrary measure spaces as follows.

\begin{definition}
\label{def:regularized_prediction}
Let $\Omega: \mathcal{M}_+^1(S) \rightarrow \mathbb{R}$ be a lower semi-continuous (l.s.c.), proper, strictly convex function,  $\mathcal{G}$ the set of measurable functions from $S$ to $\mathbb{R}$, and
\begin{equation}
  \mathcal{F} =\{ f \in \mathcal{G}: \mathbb{E}_{p}[f(t)] < \infty, \;\; \forall p\in \mathcal{M}_+^1(S) \}.\label{eq:proper}
\end{equation}
The $\Omega$-\textbf{regularized prediction map} ($\Omega-$RPM) \\ $\hat{p}_{\Omega}: \mathcal{F} \rightarrow \mathcal{M}_+^1(S)$ is defined as
\begin{equation}\label{eq:reg_prediction}
\hat{p}_{\Omega}[f] = \arg\max_{p \in \mathcal{M}_+^1(S)} \mathbb{E}_{p}[f(t)] - \Omega(p).
\end{equation}
\end{definition}

In App.~\ref{sec:appendix_existence}, we show that \eqref{eq:reg_prediction} is well defined: there is one and only one maximizer.

It is often convenient to consider a factor $\tau>0$, interpretable as a temperature,  absorbed into $\Omega$ via $\Omega := \tau \tilde{\Omega}$. If $f$ has a unique global maximizer $ t^\star $, the low-temperature limit yields ${ \lim_{\tau\rightarrow 0}}\, \hat{p}_{\Omega}[f] = \delta_{t^\star}$,
a Dirac delta distribution at the maximizer of $f$. This extends the {\bf argmax} transformation in \citet{blondel2020learning}. 
More interesting examples of regularization functionals are shown in the next subsections.

For the Shannon's negentropy $\Omega(p) = \int_S p(t)\log p(t)$, the corresponding $\Omega$-RPM recovers Boltzmann-Gibbs distributions, as shown in... \andre{Shannon entropy gives the examples shown earlier}

\andre{linear $f$ gives exponential families}

\andre{Tsallis entropy with discrete case gives sparsemax and entmax shown earlier}

\andre{recent work in ML used Tsallis entropy regularization to obtain sparse alternatives to softmax, namely entmax and sparsemax. They all work in the discrete case}

\andre{linear $f$ gives $q$-exponential families}


\subsection{Continuous sparsemax}

examples: truncated parabola, truncated paraboloid, triangular (maybe in a joint table)

example: location-scale families

\citet{blondel2020learning}  showed that, for finite $S$,  $\Omega_2$-RPM is the {\bf sparsemax} transformation, $\hat{p}_\Omega[f] = \mathrm{sparsemax}(f) =
\arg\min_{p \in \triangle} \|p - f\|^2$
(Euclidean projection of  $f\in\mathbb{R}^{|S|}$ onto the $|S|$-dimensional probability simplex $\triangle$). Other values of $\alpha$ were studied by \citet{peters2019sparse}, under the name {\bf $\alpha$-entmax} transformation. For $\alpha>1$, these transformations tend to return sparse distributions, where several entries have zero probability. This raises the question of whether similar properties can be obtained when $S$ is continuous. The following proposition (proof in  App.~\ref{sec:gini_ent_sparse_family}) answers this question by providing a general expression for $\Omega_{\alpha}$-RPM.  A key observation is that $\Omega_{\alpha}$ is strictly convex, for any $\alpha > 0$, thus satisfying the condition in Def.~\ref{def:regularized_prediction}.

\vspace{0.15cm}
\begin{proposition}\label{prop:solution_rpm_tsallis}
For $\alpha > 0$ and $f\in\mathcal{F}$, 
\begin{equation}\label{eq:entmax}
\hat{p}_{\Omega_\alpha}[f](t) =  [(\alpha - 1)(f(t) - \lambda)]_+^{1/(\alpha - 1)},
\end{equation}
where $\lambda$ is a coefficient that ensures normalization.
\end{proposition}

As shown below, for $\alpha>1$, $\hat{p}_{\Omega_\alpha}[f]$ may not have full support, \textit{i.e.}, we may have $\mathrm{supp}(\hat{p}_{\Omega_\alpha}[f]) \subsetneq S$.\footnote{This should not be confused with sparsity-inducing distributions \citep{FigueiredoNIPS2001,TippingJMLR2001}. In this paper, we say that $\mathrm{supp}(p)$ is sparse if $\nu(S \setminus \mathrm{supp}(p)) > 0$.}
Furthermore, the support may be a function of $f$, thus not constant. 

%\subsection{The 2-Tsallis entropy}

Plugging $\alpha=2$ in \eqref{eq:entmax} leads to the $\Omega_2$-RPM,
\begin{equation}\label{eq:sparsemax}
\hat{p}_{\Omega_2}[f](t) = [f(t) - \lambda]_+,
\end{equation}
\textit{i.e.}, $\hat{p}_{\Omega_2}[f]$ is obtained from $f$ by subtracting a constant (which may be negative) and truncating, where that constant $\lambda$ must be such that $ \int_S [f(t) - \lambda]_+ = 1$.

If $S$ is continuous and $\nu$ the Lebesgue measure, we call $\Omega_2$-RPM the {\bf continuous sparsemax} transformation. Some examples follow, which correspond to novel distributions.

\begin{figure*}[t]
\centering \includegraphics[width=1\textwidth]{figures/sparse_distributions}
\caption{Some location-scale families with different $\alpha$-Tsallis regularizations. Left: Gaussian and truncated parabola distributions with zero mean and different variances. Middle: same for Laplace and triangular distributions. Right: Distributions $\hat{p}_{\Omega_\alpha}[-t^2/2]$ for varying $\alpha$. \label{fig:gaussian_laplacian_distributions}}
\end{figure*}



\begin{example}\label{ex:TP} If $f(t) = -\frac{(t-\mu)^2}{2\sigma^2}$, we obtain the continuous sparsemax counterpart of a Gaussian, which we dub a ``truncated parabola,''
\begin{equation}\label{eq:truncated_parabola}
\hat{p}_{\Omega_2}[f](t) 
= \left[ - \frac{(t-\mu)^2}{2\sigma^2} - \lambda \right]_+
\eqqcolon \mathrm{TP}(t; \mu, \sigma^2),
\end{equation}
where (as shown in App.~\ref{sec:proof_truncated_parabola})
\begin{equation}\label{eq:lambda_gaussian}
\lambda = -\tfrac{1}{2}\bigl(3/(2\sigma)\bigr)^{2/3} < 0,
\end{equation}
Furthermore,  $\mathrm{supp}(\hat{p}_{\Omega_2}[f]) = [\mu - \tfrac{3}{-4\, \lambda}, \mu + \tfrac{3}{-4\, \lambda} ]$ and the 2-Tsallis negentropy is $\Omega_2(\hat{p}_{\Omega_2}[f]) = -\tfrac{1}{2} - \tfrac{2\, \lambda}{5}.$

This function, depicted in Fig.~\ref{fig:gaussian_laplacian_distributions} (left), has been widely used in density estimation, where, for $\mu=0$ and $\sigma=\sqrt{2/3}$, it is known as the Epanechnikov kernel \citep{epanechnikov1969non}.
\end{example}

\begin{example} The previous example can be generalized to $S=\mathbb{R}^N$, with $f(t)=-\frac{1}{2}(t-\mu)^\top\Sigma^{-1}(t-\mu)$, where $\Sigma \succ 0$, leading to a ``multivariate truncated paraboloid,'' the sparsemax counterpart of the multivariate Gaussian:
\begin{equation}\label{eq:truncated_paraboloid}
\hat{p}_{\Omega}[f](t) = \bigl[-\lambda - (t-\mu)\Sigma^{-1}(t-\mu)/2\bigr]_+.
\end{equation}
We show in App.~\ref{sec:proof_truncated_paraboloid} that
\begin{equation}
\lambda = -\Bigl(\Gamma\bigl(\tfrac{N}{2} + 2\bigr) / \sqrt{\mathrm{det}(2\pi \Sigma)}\Bigr)^{\frac{2}{2+N}},
\end{equation}
which reduces to \eqref{eq:lambda_gaussian} for $N=1$.
Notice that (unlike in the Gaussian case) setting $\Sigma$ to a diagonal matrix does not lead to a product of independent truncated parabolas.
\end{example}

\begin{example} Setting $f(t) = -|t-\mu|/b$, $b>0$,  yields the triangular distribution
\begin{equation}\label{eq:triangular}
\hat{p}_{\Omega_2}[f](t) = \Bigl[ -\lambda - \frac{|t-\mu|}{b}\Bigr]_+ \!
\eqqcolon \mathrm{Tri}(t; \mu,b),
\end{equation}
where (see App.~\ref{sec:proof_triangular}), $\lambda\! =\! -1/\sqrt{b}$,
$\mathrm{supp}(\hat{p}_{\Omega_2}[f]) = [\mu - \sqrt{b}, \mu + \sqrt{b}]$, and $\Omega_2(\hat{p}_{\Omega_2}[f]) = -\frac{1}{2} +  \frac{1}{3\sqrt{b}}.$
Fig.~\ref{fig:gaussian_laplacian_distributions} (center) depicts this distribution alongside Laplace.
\end{example}

\begin{example}[Location-scale families.] 

More generally, let
$f_{\mu, \sigma}(t) := -\frac{1}{\sigma}g'(|t-\mu|/\sigma)$ for a location parameter $\mu \in \mathbb{R}$ and a scale parameter $\sigma > 0$, where
$g:\mathbb{R}_+ \rightarrow \mathbb{R}$ is convex and continuously differentiable.
Then, we have
\begin{equation}
\hat{p}_{\Omega_2}[f](t) = \left[-\lambda - \frac{1}{\sigma}g'(|t-\mu|/\sigma)\right]_+,
\end{equation}
where $\lambda = -g'(a)/\sigma$
and $a$ is the solution of the equation $ag'(a) - g(a) + g(0) = \frac{1}{2}$ (a condition for such solution to exist is $g$ being strongly convex; see App.~\ref{sec:proof_location_scale} for a proof).  
The support of this distribution is
\begin{equation}
\mathrm{supp}(\hat{p}_{\Omega_2}[f_{\mu, \sigma}]) = [(-a+\mu)/\sigma, (a+\mu)/\sigma].
\end{equation}
This example subsumes the truncated parabola ($g(t) = t^3/6$) and the triangular distribution ($g(t) = t^2/2$). 
\end{example}


\subsection{Deformed exponential families and sparse families}\label{sec:deformed_sparse}

mention Naudts and Amari

definition and $A_\alpha$

proposition: gradient of $A_\alpha$ and convexity

examples


Def.~\ref{def:regularized_prediction} is fully general concerning the class of functions $\mathcal{F}$ from which $f$ can be chosen. In practice, it is often useful to consider finite-dimensional parametrized function classes. The simplest way to do this is via linear functions $f_{\theta}(t) = \theta^\top \phi(t)$, where $\phi(t)$ is a vector of \textit{statistics} and $\theta$ a vector of \textit{canonical parameters}. This construction underlies exponential families  \citep{barndorff2014information}, seen in.... 
In this section, we present {\bf sparse families} as an alternative to exponential families. Our definition is related to that of ``deformed exponential families" \citep{naudts2009q,sears2010generalized}, 
also referred to as $t$-exponential families \citep{ding2010t}, and $q$-exponential families \citep{matsuzoe2012geometry}.
Unlike those prior works, we are interested in the sparse, light tail scenario ($\alpha>1$), not in heavy tails.


\andre{Proposition 1 arises by applying the beta-exponential on f(t), and normalizing.}


\begin{definition}Let $\phi: S \rightarrow \mathbb{R}^M$ be a feature mapping. For $\alpha>1$, a family of probability distributions parametrized by $\theta \in \Theta \subseteq \mathbb{R}^M$ is called an {\bf $\alpha$-sparse family} if its members can be written in the form
\begin{equation}\label{eq:alpha_sparse_family}
    p_\theta(t) = \exp_{2-\alpha}(\theta^\top \phi(t) - A_\alpha(\theta)),
\end{equation}
where $A_\alpha: \Theta \rightarrow \mathbb{R}$ is a normalizing function (see App.~\ref{sec:A_alpha}):
\begin{equation}\label{eq:A_alpha}
A_\alpha(\theta) = \frac{\frac{1}{1-\alpha} + \int_S p_\theta(t)^{2-\alpha} \theta^\top \phi(t)}{\int_S p_\theta(t)^{2-\alpha}} - \frac{1}{1-\alpha}.
\end{equation}
\end{definition}

In particular, a 2-sparse family takes the form:
\begin{equation}\label{eq:sparse_family}
    p_\theta(t) = [\theta^\top \phi(t) - A_2(\theta) + 1]_+,
\end{equation}
where 
$A_2(\theta) = 1+ \Bigl(-1 + {\textstyle \int_{\mathrm{supp}(p_{\theta})} \theta^\top \phi(t)}\Bigr)/|\mathrm{supp}(p_{\theta})|$.
Note that $\theta^\top\! \phi(t)  - A_\alpha(\theta) = \log_{2-\alpha}(p_\theta(t))$ and that
$A_1(\theta) \!=\! {\displaystyle \lim_{\alpha\rightarrow 1}} A_\alpha(\theta) = \log \int_S \exp(\theta^\top \phi(t))$ is the log-partition function (see \eqref{eq:boltzmann}).



This construction is similar to the one in the previous section for a linear function $f(t):= \theta^\top \phi(t)$ and $\lambda := A_\alpha(\theta) - (\alpha-1)^{-1}$.
When $\alpha \rightarrow 1$, $\alpha$-sparse families become exponential families and they cease to be ``sparse'', in the sense that all distributions in the same family have the same support.






A relevant problem is that of characterizing $A_\alpha(\theta)$. When $\alpha=1$ (the log-partition function) its first and higher order derivatives are equal to the moments of the sufficient statistics. The following proposition\footnote{\label{footnote:escort}The statement involves the so-called ``$\beta$-escort distribution'' $\tilde{p}^{\beta}$ \citep{Tsallis1988}, which clearly satisfies $\tilde{p}^{1}(t) = p(t)$, given by
\[
\tilde{p}^{\beta}(t) := p(t)^{\beta} / \|p\|_\beta^\beta, \quad \text{where $\|p\|_\beta^\beta = \int_{S} p(t')^{\beta} d\nu(t')$}.
\]} (proved in App.~\ref{sec:proof_gradient_A}) characterizes $A_\alpha(\theta)$ for $\alpha \ne 1$; it will be used later to derive the Jacobian of entmax transformations and the gradient and Hessian of Fenchel-Young losses.


\vspace{0.3cm}

\begin{proposition}\label{prop:gradient_A}
The gradient of $A_\alpha(\theta)$ is given by
\begin{equation}\label{eq:derivative_of_partition}
    \nabla_\theta A_\alpha(\theta) = \mathbb{E}_{\tilde{p}_\theta^{2-\alpha}}[\phi(t)] = \frac{\int_{S} p_\theta(t)^{2-\alpha} \phi(t)}{\int_{S} p_\theta(t)^{2-\alpha}}.
\end{equation}
\end{proposition}

\andre{this proposition is stated as \citet[Theorem~5]{amari2011geometry}. The same ref shows that $A_\alpha(\theta)$ is convex. To do: add that to the theorem and add the proof. Our result is a bit more general: they assume theta is a minimal parametrization and the map btw theta and eta is one-to-one (their sec 3.1). We don’t make this assumption (in fact, our discrete examples use overcomplete parameterizations).}

The case $\alpha=1$ recovers a well-known result: the gradient of the log-partition function is the expectation of the sufficient statistics.



\paragraph{Examples of $\alpha$-sparse families.}
Truncated parabola distributions, for varying location $\mu$ and scale $\sigma$, are a 2-sparse family. Take $\phi(t) = [t, t^2]$ and define the canonical parameters $\theta = [\frac{\mu}{\sigma^2}, -\frac{1}{2\sigma^2}]$.
From \eqref{eq:lambda_gaussian}, we obtain
\begin{equation*}
    A_2(\theta) = -\frac{1}{2}\left(\frac{3}{2\sigma}\right)^{2/3} + \frac{\mu^2}{2\sigma^2} + 1 = \left(\frac{9\theta_2}{16}\right)^{1/3} - \frac{\theta_1^2}{4\theta_2} + 1.
\end{equation*}
Likewise, Gaussians are an exponential family with the same sufficient statistics and canonical parameters, and $A_1(\theta) = -\frac{\theta_1^2}{4\theta_2} - \frac{1}{2}\log(-2\theta_2)$.
Truncated parabola and Gaussians are both particular cases of the so-called ``$q$-Gaussian'' \citep[\S 4.1]{naudts2009q}, for $q = 2-\alpha$. 
\andre{consider replacing by \citep[\S 6]{naudts2010q}}
Fig.~\ref{fig:gaussian_laplacian_distributions} (right) shows $(2-\alpha)$-Gaussian distributions for $\alpha \in [1,2]$. 

Triangular distributions, with a fixed location $\mu$ and varying scale $b$, also form a 2-sparse family (similarly to Laplace distributions with fixed location being exponential families).
















\paragraph{Relation to the Tsallis maxent principle.}
The $\Omega$-RPM in Def.~\ref{def:regularized_prediction} exposes the known connection between Shannon's entropy and exponential families. This map can be seen as an incarnation of the free energy variational principle, if we see $-f_\theta(t) = -\theta^\top \phi(t)$ as an energy function and $\Omega$ the entropy scaled by a temperature. Another path is the maximum entropy (maxent) principle \citep{jaynes1957information}, a constrained optimization formulation of the same problem:
\begin{equation}\label{eq:constrained_maxent}
\max_{p \in \mathcal{M}_+^1(S)}  -\Omega(p), \hspace{0.5cm} \mathrm{s.t.}  \hspace{0.35cm} \mathbb{E}_{p}[\phi(t)] = b.
\end{equation}
As is well known, with $\Omega(p) = \int_S p(t) \log p(t)$, the solution has an exponential family form,
$p_{\theta}(t) = \exp(\theta^\top \phi(t) - A(\theta))$,
where $A(\theta)$  is the log-partition function.
Likewise, distributions in the $\alpha$-sparse family arise as solutions of a maxent problem, where $\Omega$ is an $\alpha$-Tsallis entropy.\footnote{Our construction differs from the one by \citet{Tsallis1988} and others, who use escort distributions in the expectation constraints.} 



\begin{table}[t]
    \caption{xxx} 
    \label{table:summary}
    \begin{small}
    %\begin{center}
    \begin{tabular}{lllllll}
    \toprule
    $S$ & $f(t)$ & name ($\alpha=1$) & def. & 
    name ($\alpha=2$) & def. & $\lambda$ \\
    \midrule 
    $[L]$ & $\theta_t$ & softmax & $\exp(\theta_t)/Z(\theta)$ & sparsemax & $[\theta_t - \lambda]_+$ & TBD\\
    $\mathbb{R}$ & $-\frac{(t-\mu)^2}{2\sigma^2}$ & Gaussian & $\mathcal{N}(t; \mu, \sigma^2)$ & 
    TP & $\left[-\frac{(t-\mu)^2}{2\sigma^2} - \lambda\right]_+$ & $-\frac{1}{2}(3/(2\sigma))^{2/3}$ \\
    $\mathbb{R}^N$ & $-\frac{1}{2}(t-\mu)^\top \Sigma^{-1}(t-\mu)$ & Multivariate Gaussian & $\mathcal{N}(t; \mu, \Sigma)$ & 
    Multivariate TP & $\left[-\frac{1}{2}(t-\mu)^\top \Sigma^{-1}(t-\mu) - \lambda\right]_+$ & $-\left( \Gamma(\frac{N}{2} + 2) / \sqrt{\det(2\pi\Sigma)}\right)^{\frac{2}{2+N}}$ \\
    \bottomrule
    \end{tabular}
%\end{center}
    \end{small}
\end{table}


\begin{comment}
\section{Sparse Families}\label{sec:sparse_families}

\subsection{Regularized prediction maps}

definition of RPM

point relation to variational free energy principle

Shannon entropy

example: softmax

example: multivariate Gaussian and Laplace (maybe in a joint table with truncated parabola and triangular)

linear $f$ gives exponential families




\subsection{Tsallis statistics}

$\beta$-log and $\beta$-exp (maybe use letter $q$)

Tsallis entropy

\subsection{Discrete case: entmax and sparsemax}

Use $\exp_{2-\alpha}$ notation

use $A_\alpha(f)$ notation instead of $\lambda$



\subsection{Continuous case}

should this be the beginning of a new section?

Continuous sparsemax

examples: truncated parabola, truncated paraboloid, triangular (maybe in a joint table)

example: location-scale families


\subsection{Deformed exponential families and sparse families}

mention Naudts and Amari

definition and $A_\alpha$

proposition: gradient of $A_\alpha$ and convexity

examples
\end{comment}






